Inverse Painting: Reconstructing The Painting Process

Given an input painting, we reconstruct a time-lapse video of how it may have been painted. We formulate this as an autoregressive image generation problem, in which an initially blank "canvas" is iteratively updated. The model learns from real artists by training on many painting videos. Our approach incorporates text and region understanding to define a set of painting "instructions" and updates the canvas with a novel diffusion-based renderer. The method extrapolates beyond the limited, acrylic style paintings on which it has been trained, showing plausible results for a wide range of artistic styles and genres.

==> sections/conclusion.tex <==
% \section{Conclusions}
\noindent \textbf{Conclusion}.
We propose \textit{Inverse Painting}, which generates time-lapse videos depicting a human-like painting process for a given painting. Our two-stage, diffusion-based approach is versatile, accommodating various styles of landscape paintings and producing a human-like painting process with high output quality.

